The Lick AGN Monitoring Project 2016: Dynamical Modeling of Velocity-Resolved H\b{eta} Lags in Luminous Seyfert Galaxies

We have modeled the velocity-resolved reverberation response of the H\b{eta} broad emission line in nine Seyfert 1 galaxies from the Lick Active Galactic Nucleus (AGN) Monitioring Project 2016 sample, drawing inferences on the geometry and structure of the low-ionization broad-line region (BLR) and the mass of the central supermassive black hole. Overall, we find that the H\b{eta} BLR is generally a thick disk viewed at low to moderate inclination angles. We combine our sample with prior studies and investigate line-profile shape dependence, such as log10(FWHM/{\sigma}), on BLR structure and kinematics and search for any BLR luminosity-dependent trends. We find marginal evidence for an anticorrelation between the profile shape of the broad H\b{eta} emission line and the Eddington ratio, when using the root-mean-square spectrum. However, we do not find any luminosity-dependent trends, and conclude that AGNs have diverse BLR structure and kinematics, consistent with the hypothesis of transient AGN/BLR conditions rather than systematic trends.

==> table_2016results.tex <==
\movetabledown=20mm
%\movetableright=65mm
\addtolength{\tabcolsep}{+1.5pt}
\begin{longrotatetable}
\begin{deluxetable*}{lccccccccccccc}
\tablecaption{BLR Model Parameter Values}
\tablehead{ 
\colhead{Parameter} &
\colhead{PG} &
\colhead{${\rm RXJ}$} &
\colhead{${\rm MCG}$} &
\colhead{${\rm NPM1G}$} &
\colhead{${\rm Mrk}$} &
\colhead{${\rm Mrk}$} &
\colhead{${\rm Mrk}$} &
\colhead{${\rm RBS}$} &
\colhead{${\rm Mrk}$} &
\colhead{${\rm RBS}$} &
\colhead{${\rm Ark}$} &
\colhead{${\rm Mrk}$} \\
[-0.12in]
\colhead{}&
\colhead{2209+184}&
\colhead{2044.0+2833}&
\colhead{+04-22-04} &
\colhead{+27.0587}&
\colhead{1048}&
\colhead{110}&
\colhead{1392}&
\colhead{1303}&
\colhead{9}&
\colhead{1917}&
\colhead{120}&
\colhead{841} \\
[-0.15in]%
}
\startdata
$\log_{10}(M_{\rm bh}/M_{\odot})$  & $7.53^{+0.19}_{-0.20}$ & $7.09^{+0.17}_{-0.17}$ & $7.59^{+0.42}_{-0.28}$ & $7.64^{+0.40}_{-0.36}$ & $7.79^{+0.44}_{-0.48}$ & $7.17^{+0.67}_{-0.26}$ & $8.16^{+0.11}_{-0.13}$ & $6.79^{+0.19}_{-0.11}$ & $7.09^{+0.22}_{-0.23}$ & $7.04^{+0.23}_{-0.35}$ & $8.26^{+0.12}_{-0.17}$ & $7.62^{+0.50}_{-0.30}$\\
$r_{\rm mean}$ (${\rm light~days}$)  & $16.27^{+1.04}_{-0.95}$ & $35.65^{+7.77}_{-6.25}$ & $9.94^{+1.17}_{-0.98}$ & $12.20^{+4.25}_{-3.48}$ & $14.23^{+7.84}_{-7.61}$ & $17.57^{+1.58}_{-1.51}$ & $56.01^{+12.02}_{-7.15}$ & $12.87^{+1.32}_{-1.19}$ & $11.77^{+3.61}_{-2.67}$ & $9.26^{+1.43}_{-1.61}$ & $19.22^{+2.56}_{-2.17}$ & $14.10^{+7.05}_{-4.40}$\\
$r_{\rm median}$ (${\rm light~days}$)  & $15.20^{+1.14}_{-1.04}$ & $28.30^{+7.46}_{-5.42}$ & $6.24^{+1.01}_{-0.87}$ & $7.19^{+2.83}_{-1.99}$ & $11.31^{+7.27}_{-6.24}$ & $13.89^{+2.03}_{-1.83}$ & $51.55^{+12.17}_{-8.62}$ & $10.10^{+1.33}_{-1.17}$ & $8.01^{+2.84}_{-1.85}$ & $5.00^{+1.28}_{-1.11}$ & $17.88^{+2.11}_{-2.40}$ & $10.59^{+5.57}_{-3.42}$\\
$r_{\rm min}$ (${\rm light~days}$)  & $2.83^{+1.35}_{-1.62}$ & $4.15^{+1.47}_{-1.08}$ & $1.05^{+0.65}_{-0.58}$ & $2.69^{+1.58}_{-0.95}$ & $3.34^{+2.98}_{-2.13}$ & $1.22^{+0.40}_{-0.44}$ & $40.63^{+10.95}_{-12.01}$ & $0.25^{+0.24}_{-0.18}$ & $2.21^{+0.81}_{-0.67}$ & $1.42^{+0.39}_{-0.40}$ & $1.16^{+1.40}_{-0.89}$ & $1.99^{+1.79}_{-1.07}$\\
$\sigma_r$ (${\rm light~days}$)  & $21.97^{+11.73}_{-8.27}$ & $54.78^{+45.45}_{-16.56}$ & $21.54^{+35.33}_{-9.70}$ & $22.04^{+17.69}_{-9.21}$ & $14.08^{+22.39}_{-8.67}$ & $46.63^{+12.43}_{-13.89}$ & $30.53^{+54.02}_{-17.62}$ & $13.55^{+3.82}_{-2.26}$ & $35.80^{+152.04}_{-18.37}$ & $26.76^{+25.43}_{-11.90}$ & $36.17^{+46.78}_{-20.77}$ & $14.68^{+14.92}_{-5.81}$\\
$\tau_{\rm mean}$ (${\rm days}$)  & $15.75^{+0.74}_{-0.77}$ & $30.24^{+4.79}_{-5.26}$ & $9.17^{+0.95}_{-0.81}$ & $10.72^{+3.14}_{-2.80}$ & $11.53^{+6.58}_{-6.02}$ & $18.76^{+1.99}_{-1.90}$ & $38.74^{+4.62}_{-4.22}$ & $13.71^{+1.30}_{-1.28}$ & $10.10^{+2.34}_{-2.15}$ & $9.02^{+1.88}_{-1.66}$ & $12.83^{+1.42}_{-1.26}$ & $13.53^{+4.60}_{-3.76}$\\
$\tau_{\rm median}$ (${\rm days}$)  & $12.95^{+0.87}_{-0.88}$ & $18.75^{+3.45}_{-3.94}$ & $5.58^{+0.81}_{-0.70}$ & $5.98^{+1.97}_{-1.55}$ & $8.24^{+6.20}_{-4.52}$ & $13.74^{+1.85}_{-1.79}$ & $34.82^{+4.66}_{-4.57}$ & $9.78^{+1.18}_{-1.08}$ & $5.63^{+1.47}_{-1.49}$ & $4.56^{+1.21}_{-1.15}$ & $10.99^{+1.49}_{-1.94}$ & $8.91^{+3.28}_{-2.46}$\\
$\beta$  & $0.88^{+0.14}_{-0.15}$ & $1.12^{+0.08}_{-0.08}$ & $1.40^{+0.20}_{-0.19}$ & $1.54^{+0.13}_{-0.13}$ & $1.12^{+0.28}_{-0.28}$ & $1.20^{+0.09}_{-0.09}$ & $1.29^{+0.51}_{-0.74}$ & $0.94^{+0.07}_{-0.07}$ & $1.44^{+0.12}_{-0.15}$ & $1.63^{+0.13}_{-0.16}$ & $0.89^{+0.09}_{-0.10}$ & $1.08^{+0.18}_{-0.16}$\\
$\theta_o$ (${\rm degrees}$)  & $29.1^{+11.4}_{-8.4}$ & $50.5^{+14.9}_{-12.2}$ & $13.6^{+6.9}_{-4.9}$ & $17.7^{+11.2}_{-9.0}$ & $30.8^{+13.8}_{-9.9}$ & $26.8^{+16.4}_{-13.2}$ & $41.2^{+5.2}_{-4.8}$ & $34.0^{+8.9}_{-10.0}$ & $44.9^{+16.7}_{-16.6}$ & $25.1^{+9.2}_{-7.4}$ & $31.9^{+7.0}_{-8.1}$ & $41.1^{+11.4}_{-10.7}$\\
$\theta_i$ (${\rm degrees}$)  & $30.2^{+8.7}_{-6.9}$ & $42.5^{+9.6}_{-8.4}$ & $11.3^{+5.8}_{-5.0}$ & $19.1^{+11.3}_{-8.5}$ & $21.5^{+9.4}_{-9.4}$ & $19.9^{+9.6}_{-11.5}$ & $25.5^{+3.4}_{-2.8}$ & $29.1^{+7.7}_{-9.0}$ & $41.5^{+11.6}_{-15.4}$ & $20.2^{+9.9}_{-3.9}$ & $13.6^{+3.4}_{-3.2}$ & $30.2^{+11.2}_{-15.3}$\\
$\kappa$  & $-0.09^{+0.12}_{-0.15}$ & $-0.20^{+0.33}_{-0.19}$ & $-0.14^{+0.44}_{-0.27}$ & $-0.14^{+0.40}_{-0.25}$ & $0.10^{+0.28}_{-0.38}$ & $-0.41^{+0.42}_{-0.06}$ & $0.26^{+0.18}_{-0.25}$ & $-0.48^{+0.05}_{-0.01}$ & $0.02^{+0.11}_{-0.11}$ & $-0.29^{+0.35}_{-0.14}$ & $0.26^{+0.18}_{-0.22}$ & $-0.23^{+0.43}_{-0.14}$\\
$\gamma$  & $1.4^{+0.4}_{-0.3}$ & $1.4^{+0.4}_{-0.3}$ & $1.6^{+0.3}_{-0.4}$ & $1.4^{+0.4}_{-0.3}$ & $1.5^{+0.3}_{-0.3}$ & $1.6^{+0.3}_{-0.4}$ & $1.5^{+0.3}_{-0.3}$ & $1.8^{+0.1}_{-0.2}$ & $1.6^{+0.3}_{-0.3}$ & $1.5^{+0.3}_{-0.3}$ & $1.7^{+0.2}_{-0.6}$ & $1.4^{+0.4}_{-0.3}$\\
$\xi$  & $0.73^{+0.16}_{-0.18}$ & $0.17^{+0.28}_{-0.12}$ & $0.43^{+0.35}_{-0.26}$ & $0.11^{+0.37}_{-0.09}$ & $0.30^{+0.42}_{-0.20}$ & $0.88^{+0.09}_{-0.19}$ & $0.25^{+0.28}_{-0.18}$ & $0.60^{+0.22}_{-0.16}$ & $0.52^{+0.21}_{-0.20}$ & $0.68^{+0.25}_{-0.35}$ & $0.02^{+0.04}_{-0.01}$ & $0.68^{+0.23}_{-0.41}$\\
$f_{\rm ellip}$  & $0.54^{+0.10}_{-0.15}$ & $0.41^{+0.32}_{-0.29}$ & $0.39^{+0.21}_{-0.18}$ & $0.44^{+0.19}_{-0.18}$ & $0.73^{+0.09}_{-0.13}$ & $0.60^{+0.15}_{-0.20}$ & $0.81^{+0.04}_{-0.06}$ & $0.18^{+0.17}_{-0.11}$ & $0.12^{+0.17}_{-0.08}$ & $0.59^{+0.14}_{-0.17}$ & $0.14^{+0.02}_{-0.03}$ & $0.33^{+0.24}_{-0.22}$\\
$f_{\rm flow}$  & $0.24^{+0.17}_{-0.16}$ & $0.22^{+0.19}_{-0.15}$ & $0.27^{+0.18}_{-0.19}$ & $0.26^{+0.18}_{-0.19}$ & $0.74^{+0.18}_{-0.19}$ & $0.66^{+0.22}_{-0.39}$ & $0.74^{+0.18}_{-0.18}$ & $0.75^{+0.17}_{-0.19}$ & $0.27^{+0.20}_{-0.18}$ & $0.59^{+0.28}_{-0.39}$ & $0.25^{+0.17}_{-0.17}$ & $0.45^{+0.36}_{-0.29}$\\
$\theta_e$ (${\rm degrees}$)  & $23.8^{+22.9}_{-16.0}$ & $33.7^{+31.8}_{-20.8}$ & $18.6^{+19.5}_{-12.6}$ & $35.8^{+34.8}_{-23.8}$ & $15.1^{+14.8}_{-10.1}$ & $13.7^{+15.5}_{-9.9}$ & $25.3^{+14.1}_{-15.4}$ & $8.3^{+8.8}_{-5.8}$ & $44.5^{+14.9}_{-27.6}$ & $20.3^{+21.1}_{-14.6}$ & $7.2^{+6.5}_{-4.8}$ & $50.8^{+19.9}_{-27.3}$\\
${\rm 'In. - Out.'}$  & $-0.40^{+0.09}_{-0.09}$ & $-0.37^{+0.17}_{-0.23}$ & $-0.55^{+0.27}_{-0.17}$ & $-0.41^{+0.25}_{-0.18}$ & $0.24^{+0.11}_{-0.09}$ & $0.30^{+0.21}_{-0.63}$ & $0.16^{+0.05}_{-0.03}$ & $0.80^{+0.11}_{-0.18}$ & $-0.59^{+0.23}_{-0.20}$ & $0.24^{+0.21}_{-0.63}$ & $-0.85^{+0.02}_{-0.03}$ & $-0.33^{+0.55}_{-0.31}$\\
$\sigma_{\rm turb}$  & $0.014^{+0.046}_{-0.012}$ & $0.008^{+0.033}_{-0.006}$ & $0.006^{+0.019}_{-0.004}$ & $0.012^{+0.046}_{-0.009}$ & $0.011^{+0.038}_{-0.009}$ & $0.011^{+0.038}_{-0.008}$ & $0.010^{+0.042}_{-0.008}$ & $0.006^{+0.016}_{-0.004}$ & $0.010^{+0.040}_{-0.008}$ & $0.011^{+0.043}_{-0.009}$ & $0.006^{+0.016}_{-0.004}$ & $0.011^{+0.049}_{-0.009}$\\
$r_{\rm out}$ $({\rm light~days})$  & $48$ & $131$ & $176$ & $114$ & $76$ & $56$ & $155$ & $70$ & $195$ & $50$ & $240$ & $88$
\enddata
\tablecomments{Median values and 68\% confidence intervals for BLR model parameters. Note that $r_\rm{out}$ is a fixed parameter, so we do not include uncertainties.
\label{tab: table2016_caramelresults}}
\end{deluxetable*}
\end{longrotatetable}
%\addtolength{\tabcolsep}{-1.5pt}

==> time_lag_table.tex <==
\begin{deluxetable*}{lcccc}
\tablecaption{Inferred Time Lag Comparison}
\tablewidth{0pt}
\setlength{\tabcolsep}{15pt}
\tablehead{
\colhead{Object} &
\colhead{$\tau_{\rm{median}}$ (\textsc{caramel})} &
\colhead{$\tau_{\rm{mean}}$ (\textsc{caramel})} &
\colhead{$\tau_{\rm{cen}}$ \citep{u2021lick}}
}
\startdata
PG 2209+184 & \pgataumedian & \pgataumean & $13.7^{+2.8}_{-2.9}$ \\
\mcga & \mcgataumedian & \mcgataumean & $13.3^{+2.4}_{-1.8}$\\
Mrk 1392 & \mrkataumedian & \mrkataumean & $26.7^{+3.5}_{-3.9}$\\
RBS 1303 & \rbsbtaumedian & \rbsbtaumean & $18.7^{+3.4}_{-4.3}$\\
RBS 1917 & \rbsataumedian & \rbsataumean & $11.9^{+4.3}_{-3.9}$\\
Mrk 841 & \mrketaumedian & \mrketaumean & $11.2^{+4.8}_{-3.5}$\\
RXJ 2044.0+2833 & \rxjataumedian & \rxjataumean & $14.4^{+1.6}_{-1.9}$\\
NPM1G+27.0587 & \npmgtaumedian & \npmgtaumean & $8.0^{+4.7}_{-4.5}$ \\
Mrk 1048 & \mrkdtaumedian & \mrkdtaumean & $7.4^{+9.7}_{-9.4}$
\enddata
\tablecomments{Inferred time lags for each source given by the mean and median, columns two and three, respectively, posterior distribution determined by our \textsc{caramel} modeling approach and reported using 68\% confidence intervals. Followed by the cross correlation (rest frame) time lag measurements determined by \citet{u2021lick} in column four.}
\label{tab:table_time_lag_comparison}
\end{deluxetable*}
